Improving the Performance of Deep Learning for Wireless Localization

Indoor localization systems are most commonly based on Received Signal Strength Indicator (RSSI) measurements of either WiFi or Bluetooth-Low-Energy (BLE) beacons. In such systems, the two most common techniques are trilateration and fingerprinting, with the latter providing higher accuracy. In the fingerprinting technique, Deep Learning (DL) algorithms are often used to predict the location of the receiver based on the RSSI measurements of multiple beacons received at the receiver. In this paper, we address two practical issues with applying Deep Learning to wireless localization -- transfer of solution from one wireless environment to another \emph{and} small size of labelled data set. First, we apply automatic hyperparameter optimization to a deep neural network (DNN) system for indoor wireless localization, which makes the system easy to port to new wireless environments. Second, we show how to augment a typically small labelled data set using the unlabelled data set. We observed improved performance in DL by applying the two techniques. Additionally, all relevant code has been made freely available.

==> tex/rationalize.tex <==
\section{Beacon Rationalization}
\label{rationalize}
Having addressed the issue of searching for the best hyperparameter, we now move our 
attention to another important problem that comes up in wireless localization --
\emph{could the same localization performance be achieved with fewer beacons/access
points?} 

ML algorithms are often prone to over fitting, i.e., the generated model is too 
specific to the given data set and cannot generalize enough to work equally well for a 
new data set. One of the ways to fix this is the process of regularization and dropout 
is on technique for regularization. Dropout is a technique in which 
nodes are randomly dropped from the network during the process of training. An in-depth
explanation of dropout is outside the scope of this paper but the topic is well
represented in literature. Dropout can be applied to both the hidden layer
and the visible layer.
In our case since we want to figure out the impact of any given iBeacon 
to the prediction accuracy of the DNN, we apply dropout to visible layer, namely
the input layer.

We study the impact of dropping beacons on mean localization error and the results are
shown in Figure~\ref{fig:dropout}.
We take each beacon and makes its RSSI value to be -200 dBm (no signal) in all samples.
We then remove
any sample for which that beacon was the only beacon from which it received signal. 
As an example, if beacon \emph{b01} (Figure~\ref{fig:residual_dataset}) is taken
out, 3 out of the 1420 samples (Table~\ref{tab:params}), are left with no RSSI 
measurements (there are three locations in which there is no signal from any 
of the iBeacons) and hence only 1417 samples are left to do the train and test (again
with a 80:20 train:test split). As expected, Figure~\ref{fig:residual_dataset} 
shows that dropping different iBeacons leads to different residual data sets.
Figure~\ref{fig:location_error} shows that most beacons do not have much impact on the 
localization error --- it either decreases accuracy (above the red line) or in some 
cases it improves accuracy (\emph{b01, b09}). We believe the improvement in 
accuracy is due to the fact that the addition of these iBeacons might have increased
interference in the environment --- the model is able to 
disambiguate better in the absence of these beacons.
There are however a few iBeacons 
(\emph{b03, b05, b13}) whose removal cause a noticeably large drop in accuracy. 
This means that these iBeacons are important in this environment for the overall
accuracy of the location prediction algorithm.

Even though dropout naturally fits into a DNN model, a similar concept could be 
applied to the CNN model used in this paper. However, we have not done further study
on this and hence cannot present any quantitative discussions.

